Causal Reasoning through Two Layers of Cognition for Improving Generalization in Visual Question Answering

Generalization in Visual Question Answering (VQA) requires models to answer questions about images with contexts beyond the training distribution. Existing attempts primarily refine unimodal aspects, overlooking enhancements in multimodal aspects. Besides, diverse interpretations of the input lead to various modes of answer generation, highlighting the role of causal reasoning between interpreting and answering steps in VQA. Through this lens, we propose Cognitive pathways VQA (CopVQA) improving the multimodal predictions by emphasizing causal reasoning factors. CopVQA first operates a pool of pathways that capture diverse causal reasoning flows through interpreting and answering stages. Mirroring human cognition, we decompose the responsibility of each stage into distinct experts and a cognition-enabled component (CC). The two CCs strategically execute one expert for each stage at a time. Finally, we prioritize answer predictions governed by pathways involving both CCs while disregarding answers produced by either CC, thereby emphasizing causal reasoning and supporting generalization. Our experiments on real-life and medical data consistently verify that CopVQA improves VQA performance and generalization across baselines and domains. Notably, CopVQA achieves a new state-of-the-art (SOTA) on PathVQA dataset and comparable accuracy to the current SOTA on VQA-CPv2, VQAv2, and VQA RAD, with one-fourth of the model size.

==> figures/causal_graphs/SKVQA.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[fill fraction/.style n args={2}{path picture={
            \fill[#1] (path picture bounding box.south west) rectangle
            ($(path picture bounding box.north west)!#2!(path picture bounding box.north east)$);}}]
\node[state, line width=1] (q) at (-1.4, 0.85) {$Q$};
\node[state, line width=1] (k) at (0,0) {$K$};
\node[state, line width=1] (v) at (-1.4,-0.85) {$V$};
\node[state, line width=1.2] (m1) at (0.7,1.2) {$S$};
\node[state, , line width=1, fill=yellow, fill fraction={white}{0.95}] (a) at (1.4, 0) {$A$};
\path (q) edge (k);
\path (v) edge (k);
\path (m1) edge[line width=1.2] (a);
\path (k) edge[line width=1.2] (m1);
% \path (q) edge[line width=1.2] (m1);
% \path (v) edge (a);
% \path (q) edge (a);
\path (k) edge[opacity=0.1] (a);
\path (k) edge[opacity=0.1] (a);
\end{tikzpicture}
\label{fig:skvqa}
\caption{Causal graph for VQA task with two mediators $\mathrm{K}$ and $\mathrm{S}$. $\mathrm{V}$: input image, $\mathrm{Q}$: input question, $\mathrm{K}$: multi-model knowledge, $\mathrm{S}$: cognitive strategy-awareness system, $\mathrm{A}$: answer}.
\hfill 
\end{figure}

==> figures/causal_graphs/SKVQA_nocaption.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[fill fraction/.style n args={2}{path picture={
            \fill[#1] (path picture bounding box.south west) rectangle
            ($(path picture bounding box.north west)!#2!(path picture bounding box.north east)$);}}]
\node[state, line width=1] (q) at (-1.4, 0.85) {$Q$};
\node[state, line width=1] (k) at (0,0) {$K$};
\node[state, line width=1] (v) at (-1.4,-0.85) {$V$};
\node[state, line width=1.2] (m1) at (0.7,1.2) {$S$};
\node[state, , line width=1, fill=yellow, fill fraction={white}{0.95}] (a) at (1.4, 0) {$A$};
\path (q) edge (k);
\path (v) edge (k);
\path (m1) edge[line width=1.2] (a);
\path (k) edge[line width=1.2] (m1);
% \path (q) edge[line width=1.2] (m1);
% \path (v) edge (a);
% \path (q) edge (a);
\path (k) edge[opacity=0.1] (a);
\path (k) edge[opacity=0.1] (a);
\end{tikzpicture}
\label{fig:skvqa}
% \caption{Causal graph for VQA task with two mediators $\mathrm{K}$ and $\mathrm{S}$. $\mathrm{V}$: input image, $\mathrm{Q}$: input question, $\mathrm{K}$: multi-model knowledge, $\mathrm{S}$: cognitive strategy-awareness system, $\mathrm{A}$: answer}.
\hfill 
\end{figure}

==> figures/causal_graphs/general_subtraction.tex <==
\begin{figure}[h!]
\raggedright
\begin{tikzpicture}[fill fraction/.style n args={2}{path picture={
            \fill[#1] (path picture bounding box.south west) rectangle
            ($(path picture bounding box.north west)!#2!(path picture bounding box.north east)$);}}]
\node[state, line width=1] (q) at (-1.4, 0.85) {$Q$};
\node[state, line width=1] (k) at (0,0) {$K$};
\node[state, line width=1] (v) at (-1.4,-0.85) {$V$};
\node[state, line width=1.2] (m1) at (0.7,1.2) {$\mathbf{S}$};
\node[state, , line width=1, fill=yellow, fill fraction={white}{0.95}] (a) at (1.4, 0) {$A$};
\path (q) edge (k);
\path (v) edge (k);
\path (m1) edge[line width=1.2] (a);
\path (k) edge[line width=1.2] (m1);
% \path (q) edge[line width=1.2] (m1);
% \path (v) edge (a);
% \path (q) edge (a);
\path (k) edge[opacity=0.1] (a);
\node[none] (none) at (0.1, -1.5) {($\mathbf{V}$, $\mathbf{Q}$) \rightarrow \mathbf{K} \rightarrow \mathbf{M_Q}\rightarrow \mathbf{A}}
\path (k) edge[opacity=0.1] (a);

\node[none] at (2.5, 0) {\Huge - };

\node[state, line width=1] (q1) at (3.4, 0.85) {$Q$};
% \node[state, line width=1, fill=lightgray] (qs) at (3, 0) {$q^*$};
\node[state, line width=1, opacity=0.1] (k1) at (4.3,0) {$K$};
\node[state, line width=1, opacity=0.1] (v1) at (3.4,-0.85) {$V$};
\node[state, line width=1, fill=yellow, fill fraction={white}{1},label=below:strong biased] (a1) at (5.6, 0) {$A$};

\path (q1) edge[opacity=0.1] (k1);
% \path (qs) edge (k1);
\path (v1) edge[opacity=0.1] (k1);
% \path (v1) edge[opacity=0.1] (a1);
\path (q1) edge (a1);
\path (k1) edge[opacity=0.1] (a1);
\node[none] (none) at (4.5, -1.5) {$\mathbf{Q}$ \rightarrow \mathbf{A}}
\path (k1) edge[opacity=0.1] (a1);
\label{fig:general_vqa}
\end{tikzpicture}
\hfill 
\end{figure}

==> figures/causal_graphs/main_method/z_cases.tex <==
\begin{figure*}
\centering
    \begin{subfigure}{0.24\linewidth}
  \centering
    \input{figures/causal_graphs/main_method/z_cases/z_vq_000}
    \label{fig:m1m2}
    \subcaption{$Z_{q}\xb000$}
  \end{subfigure}
  \begin{subfigure}{0.24\linewidth}
  \centering
    \input{figures/causal_graphs/main_method/z_cases/z_vq_001}
    \label{fig:m1m2}
    \subcaption{$Z_{vq}\xb001$}
  \end{subfigure}
  \begin{subfigure}{0.24\linewidth}
  \centering
    \input{figures/causal_graphs/main_method/z_cases/z_vq_010}
    \label{fig:m1m2}
    \subcaption{$Z_{q}\xb010$}
  \end{subfigure}
  \begin{subfigure}{0.24\linewidth}
  \centering
    \input{figures/causal_graphs/main_method/z_cases/z_vq_011}
    \label{fig:m1m2}
    \subcaption{$Z_{vq}\xb011$}
  \end{subfigure}
  \begin{subfigure}{0.24\linewidth}
  \centering
    \input{figures/causal_graphs/main_method/z_cases/z_vq_100}
    \label{fig:m1m2}
    \subcaption{$Z_{vq}\xb100$}
  \end{subfigure}
  \begin{subfigure}{0.24\linewidth}
  \centering
    \input{figures/causal_graphs/main_method/z_cases/z_vq_101}
    \label{fig:m1m2}
    \subcaption{$Z_{vq}\xb101$}
  \end{subfigure}
  \begin{subfigure}{0.24\linewidth}
  \centering
    \input{figures/causal_graphs/main_method/z_cases/z_vq_110}
    \subcaption{$Z_{vq}\xb110$}
    \label{fig:only_m2}
  \end{subfigure}
  \begin{subfigure}{0.24\linewidth}
  \centering
    \input{figures/causal_graphs/main_method/z_cases/z_vq_111}
    \subcaption{$Z_{vq}\xb111$}
    \label{fig:only_m1}
  \end{subfigure}
  \caption{Eight possible cases to formulate the answer distribution that is effected by either mediator $\mathrm{K}$ or $\mathrm{S}$, or only by the input question $q$.}
\end{figure*}

==> figures/causal_graphs/preliminaries/NIE_cases.tex <==
\begin{figure*}
\centering
  \begin{subfigure}{0.3\linewidth}
  \centering
    \input{figures/causal_graphs/preliminaries/NIE_cases/111}
    \subcaption{Only go through $\mathrm{M_1}$}
    \label{fig:only_m1}
  \end{subfigure}
  \begin{subfigure}{0.3\linewidth}
  \centering
    \input{figures/causal_graphs/preliminaries/NIE_cases/110}
    \subcaption{Only go through $\mathrm{M_2}$}
    \label{fig:only_m2}
  \end{subfigure}
  \begin{subfigure}{0.3\linewidth}
  \centering
    \input{figures/causal_graphs/preliminaries/NIE_cases/011}
    \label{fig:m1m2}
    \subcaption{Go through both $\mathrm{M_1}$ and $\mathrm{M_2}$}
  \end{subfigure}
  \caption{Indirect effect that go through either $\mathrm{M_1}$ or $\mathrm{M_2}$}
\end{figure*}

==> figures/causal_graphs/preliminaries/NIE_cases/011.tex <==
\begin{tikzpicture}
\node[state, line width=1] (M1) at (\xm*0.5, \ym) {$M_1$};
\node[state, line width=1] (M2) at (\xm*1.5, \ym) {$M_2$};
\node[state, line width=1] (X) at (0,0) {$X$};
\node[state, line width=1] (Y) at (2*\xm, 0) {$Y$};
\path (X) edge[opacity=\opaw] (Y);
\path (M1) edge[opacity=\opaw] (Y);
\path (M1) edge[line width=\boldw] (M2);
\path (M2) edge[line width=\boldw] (Y);
\path (X) edge[line width=\boldw] (M1);
\path (X) edge (M2);
\label{fig:general_vqa}
\end{tikzpicture}

==> figures/causal_graphs/preliminaries/NIE_cases/110.tex <==
\begin{tikzpicture}
\node[state, line width=1] (M1) at (\xm*0.5, \ym) {$M_1$};
\node[state, line width=1] (M2) at (\xm*1.5, \ym) {$M_2$};
\node[state, line width=1] (X) at (0,0) {$X$};
\node[state, line width=1] (Y) at (2*\xm, 0) {$Y$};
\path (X) edge[opacity=\opaw] (Y);
\path (M1) edge[opacity=\opaw] (Y);
\path (M1) edge[opacity=\opaw] (M2);
\path (M2) edge[line width=\boldw] (Y);
\path (X) edge[opacity=\opaw] (M1);
\path (X) edge[line width=\boldw] (M2);
\label{fig:general_vqa}
\end{tikzpicture}

==> figures/causal_graphs/preliminaries/NIE_cases/111.tex <==
\begin{tikzpicture}
\node[state, line width=1] (M1) at (\xm*0.5, \ym) {$M_1$};
\node[state, line width=1] (M2) at (\xm*1.5, \ym) {$M_2$};
\node[state, line width=1] (X) at (0,0) {$X$};
\node[state, line width=1] (Y) at (2*\xm, 0) {$Y$};
\path (X) edge[opacity=\opaw] (Y);
\path (M1) edge[line width=\boldw] (Y);
\path (M1) edge[opacity=\opaw] (M2);
\path (M2) edge[opacity=\opaw] (Y);
\path (X) edge[line width=\boldw] (M1);
\path (X) edge[opacity=\opaw] (M2);
\label{fig:general_vqa}
\end{tikzpicture}

==> figures/causal_graphs/preliminaries/basic_causal_graph.tex <==
\begin{tikzpicture}
\node[state, line width=1] (X) at (0,0) {$X$};
\node[state, line width=1] (Y) at (2*\xms, 0) {$Y$};
\path (X) edge (Y);
% \path (X) edge (M);
\end{tikzpicture}

==> figures/causal_graphs/preliminaries/general_2mediators.tex <==
\begin{tikzpicture}
\node[state, line width=1] (M1) at (\xms*0.4,  \xms-0.2) {\small{$M_1$}};
\node[state, line width=1] (M2) at (\xms*1.6,  \xms-0.2) {\small{$M_2$}};
\node[state, line width=1] (X) at (0,0) {$X$};
\node[state, line width=1] (Y) at (2*\xms, 0) {$Y$};
\path (X) edge (Y);
\path (M1) edge (Y);
\path (M1) edge (M2);
\path (M2) edge (Y);
\path (X) edge (M1);
\path (X) edge (M2);
% \node[state, line width=1] (q) at (-\xx, \yy) {$q$};
% \node[state, line width=1] (k) at (0,0) {\scriptsize{$Cop_1$}};
% \node[state, line width=1] (v) at (-\xx,-\yy) {$v$};
% \node[state, line width=1] (s) at (\xx/2,\yy*1.3) {\scriptsize{$Cop_2$}};
% \node[state, , line width=1, label=below:$A_{1}\text{-}111$] (a) at (\xx, 0) {$A$};
% \path (q) edge[line width=1.2, color=darkgreen] (k);
% \path (q) edge[bend left=5] (a);
% \path (v) edge[bend right=5] (a);
% \path (q) edge (s);
% \path (v) edge[line width=1.2, color=darkgreen] (k);
% % \path (v) edge[bend left=20] (s);
% \path (s) edge[line width=1.2, color=darkgreen] (a);
% \path (k) edge[line width=1.2, color=darkgreen] (s);
% \path (k) edge (a);

\end{tikzpicture}

==> figures/causal_graphs/preliminaries/general_foms_causalgraph.tex <==
\begin{figure*}
\centering
  \begin{subfigure}{0.3\linewidth}
  \centering
    \input{figures/causal_graphs/preliminaries/basic_causal_graph}
    \subcaption{Basic form of a causal relation}
    \label{fig:basic}
  \end{subfigure}
  \begin{subfigure}{0.3\linewidth}
  \centering
    \input{figures/causal_graphs/preliminaries/singlemediator}
    \subcaption{Causal relation with a single mediator $M$}
    \label{fig:1m}
  \end{subfigure}
  \begin{subfigure}{0.3\linewidth}
  \centering
    \input{figures/causal_graphs/preliminaries/general_2mediators}
    \subcaption{Causal relation with two mediators $M_1$ and $M_2$}
    \label{fig:2m}
  \end{subfigure}
  \caption{General forms of the causal graphs}
\end{figure*}

==> figures/causal_graphs/preliminaries/singlemediator.tex <==
\begin{tikzpicture}
\node[state, line width=1] (M) at (\ym-0.4, \xms-0.2) {$M$};
\node[state, line width=1] (X) at (0,0) {$X$};
\node[state, line width=1] (Y) at (2*\xms-0.4, 0) {$Y$};
\path (X) edge (Y);
\path (M) edge (Y);
\path (X) edge (M);

\end{tikzpicture}

==> figures/causal_graphs/preliminaries/three_graphs.tex <==
\begin{figure}[t]
\centering
% \subfloat[Basic form of a causal relation \label{fig:basic}]{\input{figures/causal_graphs/preliminaries/basic_causal_graph.tex}} \\
\subfloat[Mediator $M$ \label{fig:1m}]{\input{figures/causal_graphs/preliminaries/singlemediator.tex}} \quad \quad
\subfloat[Mediators $M_1$, $M_2$ \label{fig:2m}]{\input{figures/causal_graphs/preliminaries/general_2mediators.tex}} 
\caption{General forms of the causal graphs}
\end{figure}



% \begin{figure}[t]%
% \centering
% \subfigure[][A single mediator $M$ \label{fig:1m}]{%
% \input{figures/causal_graphs/preliminaries/singlemediator.tex}
% } \quad \quad
% \subfigure[][Mediators $M_1$, $M_2$ \label{fig:2m}]{%
% \input{figures/causal_graphs/preliminaries/general_2mediators.tex}
% } \quad \quad
% \subfigure[][Conventional VQA \label{fig:100}]{%
% \input{figures/main_method/vqa_convention.tex}
% }%
% \caption{General forms of the causal graphs}
% \label{fig:assignment_matrices}
% \end{figure}



==> figures/causal_impact.tex <==
% \begin{figure}
%   \begin{subfigure}{\linewidth}
%   \includegraphics[width=\linewidth]{figures/neg_selection_plot/VQA-CPv2_neg_k.pdf}\hfill
%   \caption{In VQA-CPv2 Dataset}
%   \end{subfigure}\par\medskip
%   \begin{subfigure}{\linewidth}
%   \includegraphics[width=.24\linewidth]{example-image-b}\hfill
%   \includegraphics[width=.24\linewidth]{example-image-b}\hfill
%   \includegraphics[width=.24\linewidth]{example-image-b}\hfill
%   \includegraphics[width=.24\linewidth]{example-image-b}
%   \caption{In Medical Dataset}
%   \end{subfigure}\par\medskip
%   \begin{subfigure}{\linewidth}
%   \includegraphics[width=.24\linewidth]{example-image-c}\hfill
%   \includegraphics[width=.24\linewidth]{example-image-c}\hfill
%   \includegraphics[width=.24\linewidth]{example-image-c}\hfill
%   \includegraphics[width=.24\linewidth]{example-image-c}
%   \caption{In CLEVR Dataset}
%   \end{subfigure}
%   \caption{Verify the causal impact of strategy selection. The \textit{Prediction} values indicate results from the selected strategy by the \textit{Guiding model}, while the \textit{Random} values represent a random selection of strategy.}
% \end{figure}


% \begin{figure}
% \centering
% \subfloat[VQA-CPv2 Dataset]{
% \centering \includegraphics[width=\linewidth]{figures/neg_selection_plot/VQA-CPv2_neg_k.pdf}
% } \quad
% \subfloat[VQAv2]{
% \centering \includegraphics[width=\linewidth]{figures/neg_selection_plot/VQA-CPv2_neg_k.pdf}
% } \\
% \subfloat[PathVQA]{
% \centering \includegraphics[width=\linewidth]{figures/neg_selection_plot/VQA-CPv2_neg_k.pdf}
% } \quad
% \subfloat[RAD-VQA]{
% \centering \includegraphics[width=\linewidth]{figures/neg_selection_plot/VQA-CPv2_neg_k.pdf}
% } \\
% \caption{Verify the causal impact of strategy selection. The \textit{Prediction} values indicate results from the selected strategy by the \textit{Guiding model}, while the \textit{Random} values represent a random selection of strategy.}
% \label{fig:causal_impact}
% \end{figure}





==> figures/method_intuition.tex <==
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.9\linewidth]{example-image-a}
%     \caption{\namealias}
%     \label{fig:das_intuition}
% \end{figure}


\newcommand\brainsize{0.7cm}
\newcommand\braindistance{1.5cm}
\newcommand\xlayerm{0}
\newcommand\xlayerh{2}
\newcommand\xlayerb{4.5}
\newcommand\xlayerbo{6.3}

\newcommand\ylayerm{0}
\newcommand\ylayerh{-1}
\newcommand\ylayerb{-2}

\newcommand\asmdis{0.5}
\newcommand\ashdis{0.7}

\definecolor{color1bg}{HTML}{ECD9ED}
\definecolor{color2bg}{HTML}{cdeac0}
\definecolor{color3bg}{HTML}{fcf5c7}
\definecolor{color4bg}{HTML}{edf2fb}


\begin{figure}[t!]
\centering
\begin{tikzpicture}[fill fraction/.style n args={2}{path picture={
            \fill[#1] (path picture bounding box.south west) rectangle
            ($(path picture bounding box.north west)!#2!(path picture bounding box.north east)$);}}]

% \node[box, line width=0, fill=green, width=3] (q) at (-0.3, 0) (3,3) {};
\draw[draw=white, fill=color4bg] (0.5,-2.7) rectangle (-0.5,0.3);
\draw[draw=white, fill=color1bg] (3.5,-2.7) rectangle (0.5,0.3);
\draw[draw=white, fill=color3bg] (5.5,-2.7) rectangle (3.5,0.3);
\draw[draw=white, fill=color4bg] (7,-2.7) rectangle (5.5,0.3);

% \node[inner sep=0cm, outer sep=0cm] (brain1) at (\xlayerh, \ylayerm + 0.3){\includegraphics[width=\brainsize, height=\brainsize]{figures/brain-pink.eps}};
% \node[inner sep=0cm, outer sep=0cm] (brain2) at (\xlayerb, \ylayerm + 0.3){\includegraphics[width=\brainsize, height=\brainsize]{figures/brain.pdf}};


\draw[draw=black, fill=white] (2.7,-0) rectangle (1.2,0.6);
\node[none, line width=1] (as1_1) at (\xlayerh, \ylayerm + 0.3) {\large{$AS_1$}};
\draw[draw=black, fill=white] (5.2,-0) rectangle (3.7,0.6);
\node[none, line width=1] (as1_2) at (\xlayerb, \ylayerm + 0.3) {\large{$AS_2$}};


%AS1 list
\node[none, line width=1] (as1_1) at (\xlayerh, \ylayerm - \asmdis) {Approach 1};
\node[none, line width=1] (as1_2) at (\xlayerh, \ylayerm - 2*\asmdis) {Approach 2};
\node[none, line width=1] (as1_3) at (\xlayerh, \ylayerm - 3*\asmdis) {Approach 3};
\node[none, line width=1] (as1_4) at (\xlayerh, \ylayerm - 4*\asmdis) {Approach 4};
\node[none, line width=1] (as1_5) at (\xlayerh, \ylayerm - 5*\asmdis) {...};

%AS2 list
\node[none, line width=1] (as2_1) at (\xlayerb, \ylayerm - \ashdis) {Strategy 1};
\node[none, line width=1] (as2_2) at (\xlayerb, \ylayerm - 2*\ashdis) {Strategy 2};
\node[none, line width=1] (as2_3) at (\xlayerb, \ylayerm - 3*\ashdis) {Strategy 3};
% \node[none, line width=1] (as2_4) at (\xlayerb, \ylayerm - 4*\ashdis) {4};
% \node[none, line width=1] (as2_5) at (\xlayerb, \ylayerm - 5*\ashdis) {5};


% \node[state, line width=1, label=left:Is this a real dog or a toy dog?] (q) at (-1, -0.85) {$Q$};
% % \node[state, line width=1] (k) at (0,0) {$K$};
\node[state, line width=1, fill=white] (q) at (\xlayerm, \ylayerh) {$Q$};
\node[state, line width=1, fill=white] (v) at (\xlayerm, \ylayerb) {$V$};
\node[state, line width=1, fill=white] (a) at (\xlayerbo, \ylayerm - 3*\asmdis) {$A$};
% \node[none] (answer) at (3.2, 0) {toy};
% \node[none] (none) at (-3.5, -2) {INPUTS};
% \node[none] (none) at (3.2, -2) {OUTPUT};
% \path (v) edge (a);
% % \path (q) edge (k);
% % \path (v) edge (k);

\path (q) edge[bend right=20, color=lightgray] (as1_5);
\path (v) edge[bend right=20, color=lightgray] (as1_5);
\path (as1_5) edge[bend right=20, color=lightgray] (as2_2);
\path (as2_2) edge[bend right=20, color=lightgray] (a);

\path (q) edge[bend left=20, color=lightgray] (as1_1);
\path (v) edge[bend left=20, color=lightgray] (as1_1);
\path (as1_1) edge[bend left=20, color=lightgray] (as2_1);
\path (as2_1) edge[bend left=20, color=lightgray] (a);

\path (q) edge[bend left=10] (as1_3);
\path (v) edge[bend left=20] (as1_3);
\path (as1_3) edge[bend left=20] (as2_2);
\path (as2_2) edge[bend right=20] (a);


% \path (img) edge[dashed] (v);
% \path (a) edge[dashed] (answer);
% \node[none] (none) at (0.1, -2) {CAUSAL GRAPH \\ ($\mathbf{V}$, $\mathbf{Q}$) \rightarrow \mathbf{A}}
% \path (a) edge[dashed] (answer);
% % \path (k) edge (a);
\end{tikzpicture}
\hfill 
\caption{\namealias overview: $AS_1$ (green area) implicitly recognizes the question's purposes, and $AS_2$ (yellow area) selects a proper strategy to give the answer.}
\label{fig:das_intuition}
\end{figure}


==> tables/main_result_VQAcp.tex <==
\setlength\tabcolsep{3pt}
\begin{table*}[t]
\caption{Baselines Result (5 Seeds)}
\label{tabke:main_result}
\begin{center}
\begin{tabular}{lccccccccc}
\toprule
Test set & \multicolumn{4}{c}{VQA-CPv2 Test} && \multicolumn{4}{c}{VQAv2 val}  \\
\cline{2-5} \cline{7-10}
Method & Overall & Y/N & Num. & Other && Overall & Y/N & Num. & Other \\
\midrule
S-MRL     & 37.02$^{\pm 0.17}$ & 41.7$^{\pm 0.32}$ & 12.47$^{\pm 0.11}$ & 41.31$^{\pm 0.3}$ && 62.99$^{\pm 0.24}$ & 81.79$^{\pm 0.18}$ & 45.63$^{\pm 0.21}$ & 53.28$^{\pm 0.34}$ \\
\quad+Ours     & 37.02$^{\pm 0.17}$ & 41.7$^{\pm 0.32}$ & 12.47$^{\pm 0.11}$ & 41.31$^{\pm 0.3}$ && 62.99$^{\pm 0.24}$ & 81.79$^{\pm 0.18}$ & 45.63$^{\pm 0.21}$ & 53.28$^{\pm 0.34}$ \\
% CF-VQA (HM)   & 50.55$^{\pm 0.2}$ & 83.54$^{\pm 1.38}$ & 19.26$^{\pm 1.89}$ & 41.84$^{\pm 0.58}$ && 59.75$^{\pm 0.35}$ & 79.37$^{\pm 0.54}$ & 41.88$^{\pm 0.77}$ & 49.56$^{\pm 0.2}$ \\
CF-VQA  & 52.13$^{\pm 0.53}$ & 90.03$^{\pm 0.31}$ & 19.0$^{\pm 1.82}$ & 41.37$^{\pm 0.56}$ && 58.05$^{\pm 0.66}$ & 78.96$^{\pm 0.73}$ & 40.52$^{\pm 0.9}$ & 46.78$^{\pm 0.68}$ \\
\quad+Ours  & 52.13$^{\pm 0.53}$ & 90.03$^{\pm 0.31}$ & 19.0$^{\pm 1.82}$ & 41.37$^{\pm 0.56}$ && 58.05$^{\pm 0.66}$ & 78.96$^{\pm 0.73}$ & 40.52$^{\pm 0.9}$ & 46.78$^{\pm 0.68}$ \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}

% \begin{table*}[t]
% \caption{Baselines Result (5 Seeds)}
% \label{tabke:main_result}
% \begin{center}
% \begin{tabular}{clccccc}
% \toprule
% Dataset & Method & Base model & Overall & Y/N & Num. & Other \\ \hline
% \multirow{4}{\rotatebox{90}{VQA-CPv2}} 
% & S-MRL    & - & 37.02$^{\pm 0.17}$ & 41.7$^{\pm 0.32}$ & 12.47$^{\pm 0.11}$ & 41.31$^{\pm 0.3}$ \\
% & \quad+Ours & - & 37.02$^{\pm 0.17}$ & 41.7$^{\pm 0.32}$ & 12.47$^{\pm 0.11}$ & 41.31$^{\pm 0.3}$ \\
% & CF-VQA  & - & 52.13$^{\pm 0.53}$ & 90.03$^{\pm 0.31}$ & 19.0$^{\pm 1.82}$ & 41.37$^{\pm 0.56}$ \\
% & \quad+Ours  & - & 52.13$^{\pm 0.53}$ & 90.03$^{\pm 0.31}$ & 19.0$^{\pm 1.82}$ & 41.37$^{\pm 0.56}$ \\ \hline
% \multirow{4}{\rotatebox{90}{VQAv2}} 
% & S-MRL    & - & 37.02$^{\pm 0.17}$ & 41.7$^{\pm 0.32}$ & 12.47$^{\pm 0.11}$ & 41.31$^{\pm 0.3}$ \\
% & \quad+Ours & - & 37.02$^{\pm 0.17}$ & 41.7$^{\pm 0.32}$ & 12.47$^{\pm 0.11}$ & 41.31$^{\pm 0.3}$ \\
% & CF-VQA  & - & 52.13$^{\pm 0.53}$ & 90.03$^{\pm 0.31}$ & 19.0$^{\pm 1.82}$ & 41.37$^{\pm 0.56}$ \\
% & \quad+Ours  & - & 52.13$^{\pm 0.53}$ & 90.03$^{\pm 0.31}$ & 19.0$^{\pm 1.82}$ & 41.37$^{\pm 0.56}$ \\ \hline
% \multirow{4}{\rotatebox{90}{VQA-CPv2}} 
% & S-MRL    & - & 37.02$^{\pm 0.17}$ & 41.7$^{\pm 0.32}$ & 12.47$^{\pm 0.11}$ & 41.31$^{\pm 0.3}$ \\
% & \quad+Ours & - & 37.02$^{\pm 0.17}$ & 41.7$^{\pm 0.32}$ & 12.47$^{\pm 0.11}$ & 41.31$^{\pm 0.3}$ \\
% & CF-VQA  & - & 52.13$^{\pm 0.53}$ & 90.03$^{\pm 0.31}$ & 19.0$^{\pm 1.82}$ & 41.37$^{\pm 0.56}$ \\
% & \quad+Ours  & - & 52.13$^{\pm 0.53}$ & 90.03$^{\pm 0.31}$ & 19.0$^{\pm 1.82}$ & 41.37$^{\pm 0.56}$ \\ \hline
% \multirow{4}{\rotatebox{90}{VQA-CPv2}} 
% & S-MRL    & - & 37.02$^{\pm 0.17}$ & 41.7$^{\pm 0.32}$ & 12.47$^{\pm 0.11}$ & 41.31$^{\pm 0.3}$ \\
% & \quad+Ours & - & 37.02$^{\pm 0.17}$ & 41.7$^{\pm 0.32}$ & 12.47$^{\pm 0.11}$ & 41.31$^{\pm 0.3}$ \\
% & CF-VQA  & - & 52.13$^{\pm 0.53}$ & 90.03$^{\pm 0.31}$ & 19.0$^{\pm 1.82}$ & 41.37$^{\pm 0.56}$ \\
% & \quad+Ours  & - & 52.13$^{\pm 0.53}$ & 90.03$^{\pm 0.31}$ & 19.0$^{\pm 1.82}$ & 41.37$^{\pm 0.56}$ \\ \hline
% \multirow{4}{\rotatebox{90}{VQA-CPv2}} 
% & S-MRL    & - & 37.02$^{\pm 0.17}$ & 41.7$^{\pm 0.32}$ & 12.47$^{\pm 0.11}$ & 41.31$^{\pm 0.3}$ \\
% & \quad+Ours & - & 37.02$^{\pm 0.17}$ & 41.7$^{\pm 0.32}$ & 12.47$^{\pm 0.11}$ & 41.31$^{\pm 0.3}$ \\
% & CF-VQA  & - & 52.13$^{\pm 0.53}$ & 90.03$^{\pm 0.31}$ & 19.0$^{\pm 1.82}$ & 41.37$^{\pm 0.56}$ \\
% & \quad+Ours  & - & 52.13$^{\pm 0.53}$ & 90.03$^{\pm 0.31}$ & 19.0$^{\pm 1.82}$ & 41.37$^{\pm 0.56}$ \\ \hline
% \end{tabular}
% \end{center}
% \end{table*}
